Improving Time Series Classification Algorithms Using Octave-Convolutional Layers

Deep learning models utilizing convolution layers have achieved state-of-the-art performance on univariate time series classification tasks. In this work, we propose improving CNN based time series classifiers by utilizing Octave Convolutions (OctConv) to outperform themselves. These network architectures include Fully Convolutional Networks (FCN), Residual Neural Networks (ResNets), LSTM-Fully Convolutional Networks (LSTM-FCN), and Attention LSTM-Fully Convolutional Networks (ALSTM-FCN). The proposed layers significantly improve each of these models with minimally increased network parameters. In this paper, we experimentally show that by substituting convolutions with OctConv, we significantly improve accuracy for time series classification tasks for most of the benchmark datasets. In addition, the updated ALSTM-OctFCN performs statistically the same as the top two time series classifers, TS-CHIEF and HIVE-COTE (both ensemble models). To further explore the impact of the OctConv layers, we perform ablation tests of the augmented model compared to their base model.

==> tables/sota.tex <==
\begin{longtable}{|c|c|c|c|c|c|c|c|c|c|}
% \tiny
 \caption{Time Series Classification Accuracy for the benchmark datasets}
  \label{results_long}


\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Dataset}               & \textbf{FCN} & \textbf{OctFCN} & \textbf{ResNet} & \textbf{OctResNet} & \textbf{LSTM-FCN} & \textbf{LSTM-OctFCN} & \textbf{ALSTM-FCN} & \textbf{ALSTM-OctFCN} & \textbf{SOTA} \\ \hline
Adiac                          & 0.768        & 0.801           & \textbf{0.833}           & 0.828              & 0.826             & 0.823                & 0.811              & 0.821                 & 0.857 \cite{wang2017time}         \\ \hline
ArrowHead                      & 0.816        & 0.855           & 0.813           & 0.846              & 0.869             & 0.884                & 0.813              & 0.868                 & \textbf{0.880} \cite{wang2017time}         \\ \hline
ChlorineConcentration          & 0.800        & 0.800           & 0.817           & 0.813              & 0.800             & 0.811                & 0.798              & 0.807                 & \textbf{0.875} \cite{wang2019time}         \\ \hline
InsectWingbeatSound            & 0.382        & 0.451           & 0.448           & 0.541              & 0.649             & 0.654                & 0.385              & 0.454                 & \textbf{0.653} \cite{bagnall2015time}         \\ \hline
Lighting7                      & 0.740        & 0.814           & 0.703           & 0.784              & 0.745             & 0.775                & 0.749              & 0.814                 & \textbf{0.863} \cite{wang2017time}         \\ \hline
Wine                           & 0.596        & 0.778           & 0.759           & 0.681              & 0.672             & 0.770                & 0.717              & 0.756                 & \textbf{0.889} \cite{wang2017time}         \\ \hline
WordsSynonyms                  & 0.532        & 0.607           & 0.609           & 0.655              & 0.657             & 0.668                & 0.544              & 0.608                 & \textbf{0.779} \cite{lines2015time}         \\ \hline
50words                        & 0.656        & 0.694           & 0.683           & 0.722              & 0.781             & 0.801                & 0.659              & 0.696                 & \textbf{0.846 } \cite{shifaz2020ts}        \\ \hline
Beef                           & 0.747        & 0.680           & 0.773           & 0.757              & 0.803             & 0.757                & 0.763              & 0.720                 & \textbf{0.933} \cite{dempster2020rocket}         \\ \hline
DistalPhalanxOutlineAgeGroup   & 0.799        & 0.799           & 0.805           & 0.785              & 0.823             & 0.807                & 0.825              & 0.816                 & \textbf{0.835} \cite{wang2017time}         \\ \hline
DistalPhalanxOutlineCorrect    & 0.803        & 0.800           & 0.798           & 0.790              & 0.803             & 0.798                & 0.801              & 0.794                 & \textbf{0.820} \cite{wang2017time}         \\ \hline
DistalPhalanxTW                & 0.776        & 0.764           & 0.766           & 0.762              & 0.779             & 0.767                & 0.783              & 0.771                 & \textbf{0.790} \cite{wang2017time}         \\ \hline
ECG200                         & 0.876        & 0.900           & 0.892           & 0.907              & 0.884             & 0.899                & 0.891              & 0.898                 & \textbf{0.920} \cite{wang2017time}         \\ \hline
ECGFiveDays                    & 0.989        & 0.993           & 0.980           & 0.991              & 0.985             & 0.990                & 0.986              & 0.993                 & \textbf{1.000} \cite{schafer2017fast}          \\ \hline
BeetleFly                      & 0.810        & 0.855           & 0.850           & 0.850              & 0.860             & 0.900                & 0.785              & 0.850                 & \textbf{0.950} \cite{schafer2017fast}         \\ \hline
BirdChicken                    & 0.935        & 0.915           & 0.925           & 0.910              & 0.900             & 0.900                & 0.935              & 0.910                 & \textbf{0.950} \cite{schafer2015boss}         \\ \hline
ItalyPowerDemand               & 0.959        & 0.956           & 0.961           & 0.958              & 0.959             & 0.956                & 0.959              & 0.956                 & \textbf{0.970 } \cite{wang2017time}        \\ \hline
SonyAIBORobotSurface           & 0.964        & 0.957           & 0.916           & 0.928              & 0.938             & 0.934                & 0.961              & 0.961                 & \textbf{0.985} \cite{wang2017time}         \\ \hline
SonyAIBORobotSurfaceII         & 0.972        & 0.965           &\textbf{ 0.980}           & 0.970              & 0.972             & 0.962                & 0.976              & 0.966                 & 0.978 \cite{baydogan2013bag}         \\ \hline
MiddlePhalanxOutlineAgeGroup   & 0.749        & 0.736           & 0.751           & 0.733              & 0.742             & 0.737                & 0.746              & 0.742                 & \textbf{0.814} \cite{baydogan2013bag}         \\ \hline
MiddlePhalanxOutlineCorrect    & \textbf{0.817}        & 0.798           & 0.816           & 0.791              & 0.814             & 0.806                & 0.816              & 0.800                 & 0.808 \cite{baydogan2013bag}         \\ \hline
MiddlePhalanxTW                & 0.585        & 0.605           & 0.595           & 0.593              & 0.595             & 0.599                & 0.594              & 0.593                 & \textbf{0.612 } \cite{wang2017time}        \\ \hline
ProximalPhalanxOutlineAgeGroup & 0.833        & 0.835           & 0.853           & 0.844              & 0.845             & 0.837                & 0.845              & 0.835                 & \textbf{0.883} \cite{bostrom2015binary}         \\ \hline
ProximalPhalanxOutlineCorrect  & 0.902        & 0.910           & 0.914           & 0.908              & 0.906             & 0.910                & 0.906              & 0.910                 & \textbf{0.918} \cite{wang2017time}         \\ \hline
ProximalPhalanxTW              & 0.811        & 0.802           & \textbf{0.816}           & 0.791              & 0.814             & 0.799                & 0.810              & 0.805                 & 0.815 \cite{schafer2015boss}         \\ \hline
MoteStrain                     & 0.918        & 0.906           & 0.909           & 0.901              & 0.927             & 0.908                & 0.920              & 0.903                 & \textbf{0.950} \cite{wang2017time}         \\ \hline
MedicalImages                  & 0.768        & 0.753           & 0.756           & 0.755              & 0.768             & 0.751                & 0.771              & 0.760                 & \textbf{0.792} \cite{wang2017time}         \\ \hline
Strawberry                     & 0.964        & 0.965           & 0.964           & 0.962              & 0.963             & 0.965                & 0.966              & 0.966                 & \textbf{0.980} \cite{schafer2015boss}        \\ \hline
ToeSegmentation1               & \textbf{0.975}        & 0.967           & 0.965           & 0.964              & 0.971             & 0.965                & 0.970              & 0.964                 & 0.974  \cite{wang2019time}       \\ \hline
Coffee                         & \textbf{1.000}        & \textbf{1.000 }          & \textbf{1.000}           & \textbf{1.000}              & \textbf{1.000}             & \textbf{1.000}                & \textbf{1.000}              & \textbf{1.000}                 & \textbf{1.000} \cite{grabocka2014learning}        \\ \hline
Cricket\_X                     & 0.773        & 0.791           & 0.788           & 0.814              & 0.746             & 0.762                & 0.782              & 0.791                 & \textbf{0.821} \cite{wang2017time}         \\ \hline
Cricket\_Y                     & 0.764        & 0.798           & 0.798           & 0.819              & 0.759             & 0.798                & 0.770              & 0.795                 & \textbf{0.826} \cite{bagnall2015time}        \\ \hline
Cricket\_Z                     & 0.774        & 0.812           & 0.804           & 0.823              & 0.786             & 0.809                & 0.783              & 0.812                 & \textbf{0.836} \cite{shifaz2020ts}         \\ \hline
uWaveGestureLibrary\_X         & 0.757        & 0.773           & 0.763           & 0.782              & 0.832             & 0.834                & 0.766              & 0.774                 & \textbf{0.855} \cite{dempster2020rocket}         \\ \hline
uWaveGestureLibrary\_Y         & 0.649        & 0.674           & 0.652           & 0.682              & 0.727             & 0.745                & 0.668              & 0.676                 & \textbf{0.759} \cite{bagnall2015time}         \\ \hline
uWaveGestureLibrary\_Z         & 0.737        & 0.745           & 0.736           & 0.747              & 0.777             & 0.773                & 0.740              & 0.745                 & \textbf{0.792} \cite{dempster2020rocket}        \\ \hline
ToeSegmentation2               & 0.903        & 0.929           & 0.899           & 0.928              & 0.905             & 0.933                & 0.905              & 0.927                 & \textbf{0.962} \cite{schafer2015boss}         \\ \hline
DiatomSizeReduction            & 0.940        & 0.930           & 0.952           & 0.933              & 0.937             & 0.937                & 0.937              & 0.936                 & \textbf{0.977} \cite{shifaz2020ts}         \\ \hline
car                            & 0.913        & 0.932           & 0.888           & 0.907              & 0.917             & 0.902                & 0.915              & 0.927                 & \textbf{0.933} \cite{wang2017time}         \\ \hline
CBF                            & 0.994        & 0.996           & 0.995           & 0.998              & 0.994             & 0.996                & 0.993              & 0.996                 & \textbf{1.000} \cite{wang2017time}         \\ \hline
CinC\_ECG\_torso               & 0.832        & 0.847           & 0.809           & 0.843              & 0.890             & 0.890                & 0.830              & 0.848                 & \textbf{0.996} \cite{dempster2020rocket}         \\ \hline
Computers                      & 0.844        & 0.832           & 0.814           & 0.814              & 0.775             & 0.734                & 0.836              & 0.828                 & \textbf{0.848} \cite{wang2017time}         \\ \hline
Earthquakes                    & 0.763        & 0.793           & 0.760           & 0.794              & 0.794             & \textbf{0.801}                & 0.783              & 0.797                 & \textbf{0.801} \cite{wang2017time}         \\ \hline
ECG5000                        & 0.939        & 0.941           & 0.940           & 0.940              & 0.942             & 0.942                & 0.940              & 0.941                 & \textbf{0.948} \cite{schafer2017fast}         \\ \hline
ElectricDevices                & 0.714        & 0.705           & 0.722           & 0.705              & 0.742             & 0.732                & 0.717              & 0.719                 & \textbf{0.799} \cite{schafer2015boss}        \\ \hline
FaceAll                        & 0.922        & 0.864           & 0.848           & 0.813              & 0.910             & 0.875                & 0.914              & 0.868                 & \textbf{0.929} \cite{wang2017time}         \\ \hline
FaceFour                       & 0.934        & 0.953           & 0.950           & 0.953              & 0.874             & 0.876                & 0.934              & 0.955                 & \textbf{1.000} \cite{schafer2017fast}         \\ \hline
FacesUCR                       & 0.933        & 0.952           & 0.942           & 0.946              & 0.917             & 0.932                & 0.934              & 0.951                 & \textbf{0.965} \cite{shifaz2020ts}         \\ \hline
Fish                           & 0.937        & 0.969           & 0.971           & 0.983              & 0.958             & 0.967                & 0.953              & 0.972                 & \textbf{0.994} \cite{shifaz2020ts}         \\ \hline
FordA                          & 0.919        & 0.924           & 0.921           & 0.928              & 0.918             & 0.931                & 0.915              & 0.924                 & \textbf{0.973} \cite{schafer2017fast}         \\ \hline
FordB                          & 0.880        & 0.902           & 0.916           & \textbf{0.918}              & 0.883             & 0.904                & 0.881              & 0.902                 & 0.917 \cite{schafer2017fast}        \\ \hline
Gun\_Point                     & \textbf{1.000}        & \textbf{1.000}           & 0.997           & \textbf{1.000}              & 0.995             & 0.998                & \textbf{1.000}              & \textbf{1.000}                 & \textbf{1.000} \cite{schafer2017fast}         \\ \hline
Ham                            & 0.715        & 0.750           & 0.712           & 0.730              & 0.717             & 0.727                & 0.720              & 0.750                 & \textbf{0.781} \cite{wang2017time}         \\ \hline
HandOutlines                   & 0.521        & 0.755           & 0.880           & 0.871              & 0.842             & 0.875                & 0.623              & 0.806                 & \textbf{0.960} \cite{wang2019time}         \\ \hline
Haptics                        & 0.426        & 0.494           & 0.517           & 0.553              & 0.489             & 0.514                & 0.465              & 0.510                 & \textbf{0.551} \cite{wang2017time}         \\ \hline
Herring                        & 0.634        & 0.703           & 0.614           & 0.661              & 0.641             & 0.698                & 0.647              & \textbf{0.727}                 & 0.703 \cite{wang2017time}        \\ \hline
InlineSkate                    & 0.374        & 0.423           & 0.482           & 0.432              & 0.465             & 0.446                & 0.424              & 0.427                 & \textbf{0.613} \cite{schafer2017fast}         \\ \hline
LargeKitchenAppliances         & 0.890        & 0.895           & \textbf{0.903}           & 0.897              & 0.685             & 0.744                & 0.897              & 0.897                 & 0.896 \cite{wang2017time}         \\ \hline
Lighting2                      & 0.708        & 0.711           & 0.730           & 0.726              & 0.752             & 0.769                & 0.718              & 0.728                 & \textbf{0.885} \cite{lines2015time}         \\ \hline
MALLAT                         & 0.963        & 0.966           & 0.938           & 0.961              & 0.963             & 0.961                & 0.966              & 0.966                 & \textbf{0.980} \cite{wang2017time}         \\ \hline
Meat                           & 0.863        & 0.875           & 0.938           & 0.942              & 0.895             & 0.922                & 0.885              & 0.910                 & \textbf{1.000} \cite{wang2017time}         \\ \hline
NonInvasiveFatalECG\_Thorax1   & 0.949        & 0.958           & 0.954           & 0.955              & \textbf{0.962}             & \textbf{0.962}                 & 0.955              & 0.956                 & \textbf{0.962} \cite{wang2019time}         \\ \hline
NonInvasiveFatalECG\_Thorax2   & 0.929        & 0.947           & 0.949           & 0.956              & 0.954             & 0.957                & 0.948              & 0.951                 & \textbf{0.969 } \cite{dempster2020rocket}       \\ \hline
OliveOil                       & 0.533        & 0.720           & 0.827           & 0.847              & 0.593             & 0.770                & 0.587              & 0.767                 & \textbf{0.933} \cite{schafer2017fast}          \\ \hline
OSULeaf                        & 0.979        & 0.970           & 0.974           & 0.965              & 0.895             & 0.907                & 0.979              & 0.971                 & \textbf{0.988} \cite{wang2017time}         \\ \hline
PhalangesOutlinesCorrect       & 0.813        & 0.821           & 0.825           & 0.821              & 0.816             & 0.817                & 0.812              & 0.817                 & \textbf{0.854} \cite{wang2019time}         \\ \hline
Phoneme                        & 0.336        & 0.345           & \textbf{0.354}           & 0.345              & 0.252             & 0.265                & 0.340              & 0.343                 & 0.349 \cite{bagnall2015time}         \\ \hline
plane                          & \textbf{1.000}        & \textbf{1.000}           & \textbf{1.000 }          & \textbf{1.000}              & \textbf{1.000}             & \textbf{1.000}                & \textbf{1.000}              & \textbf{1.000}                 & \textbf{1.000} \cite{schafer2017fast}         \\ \hline
RefrigerationDevices           & 0.510        & 0.528           & 0.555           & 0.534              & 0.466             & 0.480                & 0.507              & 0.525                 & \textbf{0.581} \cite{bostrom2015binary}         \\ \hline
ScreenType                     & 0.637        & 0.637           & 0.648           & 0.627              & 0.545             & 0.510                & 0.639              & 0.634                 & \textbf{0.707 } \cite{wang2017time}        \\ \hline
ShapeletSim                    & 0.956        & 0.926           & 0.948           & 0.874              & 0.966             & 0.953                & 0.927              & 0.921                 & \textbf{1.000} \cite{schafer2017fast}         \\ \hline
ShapesAll                      & 0.885        & 0.903           & 0.912           & 0.917              & 0.890             & 0.904                & 0.884              & 0.902                 & \textbf{0.930} \cite{shifaz2020ts}         \\ \hline
SmallKitchenAppliances         & 0.734        & 0.759           & 0.769           & 0.735              & 0.610             & 0.599                & 0.766              & 0.757                 & \textbf{0.853} \cite{dempster2020rocket}         \\ \hline
StarlightCurves                & 0.964        & 0.975           & 0.976           & 0.977              & 0.965             & 0.974                & 0.964              & 0.975                 & \textbf{0.982} \cite{shifaz2020ts}         \\ \hline
SwedishLeaf                    & 0.969        & 0.966           & 0.960           & 0.960              & \textbf{0.971}             & 0.968                & 0.968              & 0.968                 & 0.966 \cite{schafer2017fast}         \\ \hline
Symbols                        & 0.973        & \textbf{0.983 }          & 0.972           & 0.980              & 0.963             & 0.963                & 0.976              & 0.984                 & 0.982 \cite{wang2019time}         \\ \hline
synthetic\_control             & 0.985        & 0.999           & 0.994           & 0.998              & 0.978             & 0.999                & 0.980              & 0.999                 & \textbf{1.000} \cite{lines2015time}         \\ \hline
Trace                          & 0.250        & 0.250           & 0.250           & 0.250              & 0.250             & 0.250                & 0.250              & 0.250                 & \textbf{1.000 } \cite{schafer2017fast}        \\ \hline
Two\_Patterns                  & 0.863        & 0.942           & 0.963           & 0.991              & 0.994             & 0.984                & 0.873              & 0.943                 & \textbf{1.000} \cite{dempster2020rocket}        \\ \hline
TwoLeadECG                     & 0.999        & 0.998           & 0.999           & 0.996              & 0.999             & 0.998                & 0.999              & 0.998                 & \textbf{1.000} \cite{lines2015time}         \\ \hline
UWaveGestureLibraryAll         & 0.822        & 0.864           & 0.833           & 0.874              & 0.955             & 0.959                & 0.824              & 0.861                 & \textbf{0.976} \cite{dempster2020rocket}        \\ \hline
wafer                          & 0.997        & 0.999           & 0.995           & 0.997              & 0.998             & 0.999                & 0.997              & 0.998                 & \textbf{1.000 } \cite{schafer2017fast}        \\ \hline
Worms                          & 0.612        & 0.650           & 0.598           & 0.626              & 0.494             & 0.534                & 0.606              & 0.651                 & \textbf{0.805} \cite{schafer2017fast}         \\ \hline
WormsTwoClass                  & 0.773        & 0.774           & 0.771           & 0.762              & 0.683             & 0.699                & 0.781              & 0.773                 & \textbf{0.831} \cite{bostrom2015binary}         \\ \hline
yoga                           & 0.860        & 0.879           & 0.878           & 0.888              & 0.903             & 0.904                & 0.879              & 0.883                 & \textbf{0.918} \cite{schafer2015boss}        \\ \hline
ACSF1            & 0.927        & 0.935           & 0.917           & 0.932              & 0.903             & 0.920                & 0.913              & \textbf{0.940}                 & 0.850 \cite{lines2018time}         \\ \hline
AllGestWiX       & 0.615        & 0.646           & 0.707           & 0.718              & 0.693             & \textbf{0.724}                & 0.718              & 0.722                 & 0.717 \cite{bagnall2018uea}        \\ \hline
AllGestWiY       & 0.746        & 0.778           & 0.764           & 0.773              & 0.753             & 0.781                & 0.788              & \textbf{0.856}                 & 0.730 \cite{bagnall2018uea}        \\ \hline
AllGestWiZ       & 0.694        & 0.725           & 0.715           & 0.720              & 0.704             & \textbf{0.758}                & 0.733              & 0.746                 & 0.651 \cite{bagnall2018uea}        \\ \hline
BME              & 0.947        & 0.980           & 0.953           & 0.968              & 0.952             & 0.996                & 0.833              & 0.900                 & \textbf{0.999} \cite{lines2018time}        \\ \hline
Chinatown        & 0.938        & 0.956           & 0.964           & 0.973              & 0.988             & 0.988                & 0.985              & \textbf{0.995}                 & 0.970 \cite{lines2018time}        \\ \hline
Crop             & 0.764        & 0.783           & 0.789           & 0.793              & 0.764             & \textbf{0.875}                & 0.762              & 0.799                 & 0.793 \cite{wang2019time}        \\ \hline
DodgLpDay        & 0.614        & 0.647           & 0.647           & 0.648              & 0.634             & \textbf{0.652}                & 0.486              & 0.550                 & 0.588 \cite{bagnall2018uea}        \\ \hline
DodgLpGm         & 0.826        & 0.833           & 0.846           & 0.856              & 0.893             & 0.907                & 0.779              & 0.823                 & \textbf{0.928} \cite{bagnall2018uea}        \\ \hline
DodgLpWnd        & 0.938        & 0.967           & 0.949           & 0.949              & 0.927             & 0.933                & 0.970              & 0.973                 & \textbf{0.986} \cite{bagnall2018uea}        \\ \hline
EOGHzSgn         & 0.651        & 0.656           & 0.652           & 0.663              & 0.617             & 0.632                & 0.686              & 0.680                 & \textbf{0.884} \cite{wang2019time}         \\ \hline
EOGVtSgn         & 0.473        & 0.490           & 0.465           & 0.472              & 0.504             & 0.529                & 0.514              & 0.518                 & \textbf{0.815} \cite{wang2019time}         \\ \hline
EthLevel         & 0.737        & 0.743           & 0.753           & 0.737              & 0.725             & 0.763                & 0.738              & 0.727                 & \textbf{0.875} \cite{wang2019time}         \\ \hline
FrzRegTr         & 0.957        & 0.991           & 0.970           & 0.965              & 0.998             & \textbf{1.000}                & \textbf{1.000}              & \textbf{1.000}                 & 0.999 \cite{shifaz2020ts}         \\ \hline
FRSmlTr          & 0.829        & 0.842           & 0.816           & 0.822              & 0.807             & 0.836                & 0.878              & 0.897                 & \textbf{0.995} \cite{shifaz2020ts}         \\ \hline
Fungi            & 0.983        & 0.998           & 0.994           & 0.996              & 0.984             & \textbf{1.000}                & 0.995              & \textbf{1.000}                 & 0.839 \cite{bagnall2018uea}        \\ \hline
GestMidAirD1     & 0.736        & 0.742           & 0.719           & 0.746              & 0.703             & \textbf{0.751}                & 0.714              & \textbf{0.751}                 & 0.639 \cite{bagnall2018uea}        \\ \hline
GestMidAirD2     & 0.672        & 0.677           & 0.657           & 0.669              & \textbf{0.694}             & 0.681                & 0.640              & 0.628                 & 0.608 \cite{bagnall2018uea}        \\ \hline
GestMidAirD3     & 0.421        & 0.440           & 0.390           & 0.433              &\textbf{ 0.452}             & 0.433                & 0.444              & 0.435                 & 0.377 \cite{bagnall2018uea}        \\ \hline
GestPebZ1        & 0.944        & \textbf{0.973}           & 0.941           & 0.949              & 0.947             & 0.933                & 0.921              & 0.921                 & 0.826 \cite{bagnall2018uea}        \\ \hline
GestPebZ2        & 0.857        & 0.883           & 0.892           & 0.864              & 0.873             & \textbf{0.913}                & 0.832              & 0.818                 & 0.779 \cite{bagnall2018uea}        \\ \hline
GunPtAgeSp       & 0.982        & 0.973           & 0.998           & 0.995              & 0.986             & 0.988                & \textbf{1.000 }             & 0.970                 & \textbf{1.000} \cite{shifaz2020ts}         \\ \hline
GunPontMVsF      & 0.962        & 0.987           & 0.976           & 0.957              & 0.980             & 0.989                & \textbf{1.000}              & \textbf{1.000}                 & \textbf{1.000} \cite{lines2018time}        \\ \hline
GunPointOVsY     & 0.942        & 0.949           & 0.995           & 0.957              & 0.974             & 0.983                & \textbf{1.000}              & 0.986                 & \textbf{1.000} \cite{shifaz2020ts}         \\ \hline
HouseTwenty      & 0.945        & 0.955           & 0.908           & 0.961              & 0.970             & 0.962                & 0.948              & 0.970                 & \textbf{0.979} \cite{lines2018time}        \\ \hline
InsEPGRegTr      & \textbf{1.000}        & \textbf{1.000}           & \textbf{1.000}           & 0.995              & \textbf{1.000}             & 0.994                & \textbf{1.000}              & 0.991                 & \textbf{1.000 } \cite{shifaz2020ts}        \\ \hline
InsEPGSmlTr      & 0.928        & 0.958           & \textbf{1.000}           & 0.920              & \textbf{1.000}             & 0.981                & \textbf{1.000}              & 0.976                 & \textbf{1.000} \cite{shifaz2020ts}         \\ \hline
MelbPed          & 0.972        & \textbf{0.993}           & 0.983           & 0.988              & 0.973             & 0.951                & 0.976              & 0.979                 & 0.848 \cite{bagnall2018uea}        \\ \hline
MxShpRegTr       & 0.928        & 0.942           & 0.975           & 0.984              & 0.963             & \textbf{0.991}                & 0.968              & 0.981                 & 0.971 \cite{shifaz2020ts}         \\ \hline
MxShpSmlTr       & 0.918        & 0.941           & 0.928           & 0.936              & 0.922             & 0.927                & 0.924              & 0.915                 & \textbf{0.947} \cite{shifaz2020ts}         \\ \hline
PickGestWiZ      & 0.853        & 0.878           & 0.864           & 0.851              & 0.897             & 0.895                & 0.899              & \textbf{0.900}                 & 0.660 \cite{bagnall2018uea}        \\ \hline
PigAryPress      & 0.750        & 0.760           & 0.753           & 0.740              & 0.793             & 0.824                & 0.756              & 0.826                 & \textbf{0.977} \cite{wang2019time}         \\ \hline
PigArtPress      & 0.964        & 0.974           & 0.974           & 0.977              & 0.985             & \textbf{1.000}                & 0.995              & \textbf{1.000}                 & 0.975 \cite{wang2019time}         \\ \hline
PigCVP           & 0.864        & 0.869           & 0.871           & 0.937              & 0.922             & 0.941                & 0.928              & 0.956                 & \textbf{0.961} \cite{shifaz2020ts}         \\ \hline
PLAID            & 0.481        & 0.489           & 0.482           & 0.494              & 0.282             & 0.483                & 0.506              & 0.515                 & \textbf{0.840} \cite{bagnall2018uea}        \\ \hline
PowerCons        & 0.973        & 0.984           & 0.973           & 0.981              & \textbf{1.000}             & \textbf{1.000}                & 0.984              & \textbf{1.000}                 & 0.993 \cite{wang2019time}         \\ \hline
Rock             & 0.718        & 0.727           & 0.676           & 0.729              & 0.764             & 0.782                & 0.795              & 0.805                 & \textbf{0.867} \cite{wang2019time}         \\ \hline
SgHdGendCh2      & 0.943        & 0.969           & 0.937           & 0.959              & 0.945             & \textbf{0.986}                & 0.852              & 0.879                 & 0.969 \cite{lines2018time}        \\ \hline
SgHdMovCh2       & 0.612        & 0.626           & 0.698           & 0.630              & 0.703             & 0.714                & 0.653              & 0.716                 & \textbf{0.891} \cite{wang2019time}         \\ \hline
SgHdSubCh2       & 0.919        & 0.927           & 0.925           & 0.932              & 0.917             & 0.917                & 0.902              & 0.917                 & \textbf{0.951} \cite{lines2018time}        \\ \hline
ShkGestWiZ       & 0.961        & \textbf{0.981}           & 0.973           & 0.966              & 0.946             & 0.992                & 0.975              & 0.974                 & 0.860 \cite{bagnall2018uea}        \\ \hline
SmthSub          & 0.986        & 0.983           & 0.993           & 0.988              & \textbf{1.000}             & 0.988                & \textbf{1.000}              & \textbf{1.000 }                & 0.998 \cite{shifaz2020ts}        \\ \hline
UMB              & 0.989        & \textbf{1.000} \cite{wang2019time}           & \textbf{1.000}           & 0.982              & \textbf{1.000}             & 0.966                & 0.989              & \textbf{1.000}                 & 0.983 \cite{shifaz2020ts}        \\ \hline
\end{tabular}
\end{longtable}

==> tables/sota_new.tex <==
\begin{table*}[h]
\scriptsize
 \caption{Time Series Classification Accuracies for the newest 43 benchmark datasets}
 \label{results_2}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{FCN} & \textbf{OctFCN} & \textbf{ResNet} & \textbf{OctResNet} & \textbf{LSTM-FCN} & \textbf{LSTM-OctFCN} & \textbf{ALSTM-FCN} & \textbf{ALSTM-OctFCN} & \textbf{SOTA} \\ \hline
ACSF1            & 0.927        & 0.935           & 0.917           & 0.932              & 0.903             & 0.920                & 0.913              & 0.940                 & 0.850         \\ \hline
AllGestWiX       & 0.615        & 0.646           & 0.707           & 0.718              & 0.693             & 0.724                & 0.718              & 0.722                 & 0.717         \\ \hline
AllGestWiY       & 0.746        & 0.778           & 0.764           & 0.773              & 0.753             & 0.781                & 0.788              & 0.856                 & 0.730         \\ \hline
AllGestWiZ       & 0.694        & 0.725           & 0.715           & 0.720              & 0.704             & 0.758                & 0.733              & 0.746                 & 0.651         \\ \hline
BME              & 0.947        & 0.980           & 0.953           & 0.968              & 0.952             & 0.996                & 0.833              & 0.900                 & 0.999         \\ \hline
Chinatown        & 0.938        & 0.956           & 0.964           & 0.973              & 0.988             & 0.988                & 0.985              & 0.995                 & 0.970         \\ \hline
Crop             & 0.764        & 0.783           & 0.789           & 0.793              & 0.764             & 0.875                & 0.762              & 0.799                 & 0.793         \\ \hline
DodgLpDay        & 0.614        & 0.647           & 0.647           & 0.648              & 0.634             & 0.652                & 0.486              & 0.550                 & 0.588         \\ \hline
DodgLpGm         & 0.826        & 0.833           & 0.846           & 0.856              & 0.893             & 0.907                & 0.779              & 0.823                 & 0.928         \\ \hline
DodgLpWnd        & 0.938        & 0.967           & 0.949           & 0.949              & 0.927             & 0.933                & 0.970              & 0.973                 & 0.986         \\ \hline
EOGHzSgn         & 0.651        & 0.656           & 0.652           & 0.663              & 0.617             & 0.632                & 0.686              & 0.680                 & 0.884         \\ \hline
EOGVtSgn         & 0.473        & 0.490           & 0.465           & 0.472              & 0.504             & 0.529                & 0.514              & 0.518                 & 0.815         \\ \hline
EthLevel         & 0.737        & 0.743           & 0.753           & 0.737              & 0.725             & 0.763                & 0.738              & 0.727                 & 0.875         \\ \hline
FrzRegTr         & 0.957        & 0.991           & 0.970           & 0.965              & 0.998             & 1.000                & 1.000              & 1.000                 & 0.999         \\ \hline
FRSmlTr          & 0.829        & 0.842           & 0.816           & 0.822              & 0.807             & 0.836                & 0.878              & 0.897                 & 0.995         \\ \hline
Fungi            & 0.983        & 0.998           & 0.994           & 0.996              & 0.984             & 1.000                & 0.995              & 1.000                 & 0.839         \\ \hline
GestMidAirD1     & 0.736        & 0.742           & 0.719           & 0.746              & 0.703             & 0.751                & 0.714              & 0.751                 & 0.639         \\ \hline
GestMidAirD2     & 0.672        & 0.677           & 0.657           & 0.669              & 0.694             & 0.681                & 0.640              & 0.628                 & 0.608         \\ \hline
GestMidAirD3     & 0.421        & 0.440           & 0.390           & 0.433              & 0.452             & 0.433                & 0.444              & 0.435                 & 0.377         \\ \hline
GestPebZ1        & 0.944        & 0.973           & 0.941           & 0.949              & 0.947             & 0.933                & 0.921              & 0.921                 & 0.826         \\ \hline
GestPebZ2        & 0.857        & 0.883           & 0.892           & 0.864              & 0.873             & 0.913                & 0.832              & 0.818                 & 0.779         \\ \hline
GunPtAgeSp       & 0.982        & 0.973           & 0.998           & 0.995              & 0.986             & 0.988                & 1.000              & 0.970                 & 1.000         \\ \hline
GunPontMVsF      & 0.962        & 0.987           & 0.976           & 0.957              & 0.980             & 0.989                & 1.000              & 1.000                 & 1.000         \\ \hline
GunPointOVsY     & 0.942        & 0.949           & 0.995           & 0.957              & 0.974             & 0.983                & 1.000              & 0.986                 & 1.000         \\ \hline
HouseTwenty      & 0.945        & 0.955           & 0.908           & 0.961              & 0.970             & 0.962                & 0.948              & 0.970                 & 0.979         \\ \hline
InsEPGRegTr      & 1.000        & 1.000           & 1.000           & 0.995              & 1.000             & 0.994                & 1.000              & 0.991                 & 1.000         \\ \hline
InsEPGSmlTr      & 0.928        & 0.958           & 1.000           & 0.920              & 1.000             & 0.981                & 1.000              & 0.976                 & 1.000         \\ \hline
MelbPed          & 0.972        & 0.993           & 0.983           & 0.988              & 0.973             & 0.951                & 0.976              & 0.979                 & 0.848         \\ \hline
MxShpRegTr       & 0.928        & 0.942           & 0.975           & 0.984              & 0.963             & 0.991                & 0.968              & 0.981                 & 0.971         \\ \hline
MxShpSmlTr       & 0.918        & 0.941           & 0.928           & 0.936              & 0.922             & 0.927                & 0.924              & 0.915                 & 0.947         \\ \hline
PickGestWiZ      & 0.853        & 0.878           & 0.864           & 0.851              & 0.897             & 0.895                & 0.899              & 0.900                 & 0.660         \\ \hline
PigAryPress      & 0.750        & 0.760           & 0.753           & 0.740              & 0.793             & 0.824                & 0.756              & 0.826                 & 0.977         \\ \hline
PigArtPress      & 0.964        & 0.974           & 0.974           & 0.977              & 0.985             & 1.000                & 0.995              & 1.000                 & 0.975         \\ \hline
PigCVP           & 0.864        & 0.869           & 0.871           & 0.937              & 0.922             & 0.941                & 0.928              & 0.956                 & 0.961         \\ \hline
PLAID            & 0.481        & 0.489           & 0.482           & 0.494              & 0.282             & 0.483                & 0.506              & 0.515                 & 0.840         \\ \hline
PowerCons        & 0.973        & 0.984           & 0.973           & 0.981              & 1.000             & 1.000                & 0.984              & 1.000                 & 0.993         \\ \hline
Rock             & 0.718        & 0.727           & 0.676           & 0.729              & 0.764             & 0.782                & 0.795              & 0.805                 & 0.867         \\ \hline
SgHdGendCh2      & 0.943        & 0.969           & 0.937           & 0.959              & 0.945             & 0.986                & 0.852              & 0.879                 & 0.969         \\ \hline
SgHdMovCh2       & 0.612        & 0.626           & 0.698           & 0.630              & 0.703             & 0.714                & 0.653              & 0.716                 & 0.891         \\ \hline
SgHdSubCh2       & 0.919        & 0.927           & 0.925           & 0.932              & 0.917             & 0.917                & 0.902              & 0.917                 & 0.951         \\ \hline
ShkGestWiZ       & 0.961        & 0.981           & 0.973           & 0.966              & 0.946             & 0.992                & 0.975              & 0.974                 & 0.860         \\ \hline
SmthSub          & 0.986        & 0.983           & 0.993           & 0.988              & 1.000             & 0.988                & 1.000              & 1.000                 & 0.998         \\ \hline
UMB              & 0.989        & 1.000           & 1.000           & 0.982              & 1.000             & 0.966                & 0.989              & 1.000                 & 0.983         \\ \hline
\end{tabular}
\end{table*}

==> tables/sota_org.tex <==
\begin{table*}[h]
\tinytiny
 \caption{Time Series Classification Accuracies for the first 85 benchmark datasets}
  \label{results_1}


\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Dataset}               & \textbf{FCN} & \textbf{OctFCN} & \textbf{ResNet} & \textbf{OctResNet} & \textbf{LSTM-FCN} & \textbf{LSTM-OctFCN} & \textbf{ALSTM-FCN} & \textbf{ALSTM-OctFCN} & \textbf{SOTA} \\ \hline
Adiac                          & 0.768        & 0.801           & 0.833           & 0.828              & 0.826             & 0.823                & 0.811              & 0.821                 & 0.857         \\ \hline
ArrowHead                      & 0.816        & 0.855           & 0.813           & 0.846              & 0.869             & 0.884                & 0.813              & 0.868                 & 0.880         \\ \hline
ChlorineConcentration          & 0.800        & 0.800           & 0.817           & 0.813              & 0.800             & 0.811                & 0.798              & 0.807                 & 0.875         \\ \hline
InsectWingbeatSound            & 0.382        & 0.451           & 0.448           & 0.541              & 0.649             & 0.654                & 0.385              & 0.454                 & 0.653         \\ \hline
Lighting7                      & 0.740        & 0.814           & 0.703           & 0.784              & 0.745             & 0.775                & 0.749              & 0.814                 & 0.863         \\ \hline
Wine                           & 0.596        & 0.778           & 0.759           & 0.681              & 0.672             & 0.770                & 0.717              & 0.756                 & 0.889         \\ \hline
WordsSynonyms                  & 0.532        & 0.607           & 0.609           & 0.655              & 0.657             & 0.668                & 0.544              & 0.608                 & 0.779         \\ \hline
50words                        & 0.656        & 0.694           & 0.683           & 0.722              & 0.781             & 0.801                & 0.659              & 0.696                 & 0.846         \\ \hline
Beef                           & 0.747        & 0.680           & 0.773           & 0.757              & 0.803             & 0.757                & 0.763              & 0.720                 & 0.933         \\ \hline
DistalPhalanxOutlineAgeGroup   & 0.799        & 0.799           & 0.805           & 0.785              & 0.823             & 0.807                & 0.825              & 0.816                 & 0.835         \\ \hline
DistalPhalanxOutlineCorrect    & 0.803        & 0.800           & 0.798           & 0.790              & 0.803             & 0.798                & 0.801              & 0.794                 & 0.820         \\ \hline
DistalPhalanxTW                & 0.776        & 0.764           & 0.766           & 0.762              & 0.779             & 0.767                & 0.783              & 0.771                 & 0.790         \\ \hline
ECG200                         & 0.876        & 0.900           & 0.892           & 0.907              & 0.884             & 0.899                & 0.891              & 0.898                 & 0.920         \\ \hline
ECGFiveDays                    & 0.989        & 0.993           & 0.980           & 0.991              & 0.985             & 0.990                & 0.986              & 0.993                 & 1.000         \\ \hline
BeetleFly                      & 0.810        & 0.855           & 0.850           & 0.850              & 0.860             & 0.900                & 0.785              & 0.850                 & 0.950         \\ \hline
BirdChicken                    & 0.935        & 0.915           & 0.925           & 0.910              & 0.900             & 0.900                & 0.935              & 0.910                 & 0.950         \\ \hline
ItalyPowerDemand               & 0.959        & 0.956           & 0.961           & 0.958              & 0.959             & 0.956                & 0.959              & 0.956                 & 0.970         \\ \hline
SonyAIBORobotSurface           & 0.964        & 0.957           & 0.916           & 0.928              & 0.938             & 0.934                & 0.961              & 0.961                 & 0.985         \\ \hline
SonyAIBORobotSurfaceII         & 0.972        & 0.965           & 0.980           & 0.970              & 0.972             & 0.962                & 0.976              & 0.966                 & 0.978         \\ \hline
MiddlePhalanxOutlineAgeGroup   & 0.749        & 0.736           & 0.751           & 0.733              & 0.742             & 0.737                & 0.746              & 0.742                 & 0.814         \\ \hline
MiddlePhalanxOutlineCorrect    & 0.817        & 0.798           & 0.816           & 0.791              & 0.814             & 0.806                & 0.816              & 0.800                 & 0.808         \\ \hline
MiddlePhalanxTW                & 0.585        & 0.605           & 0.595           & 0.593              & 0.595             & 0.599                & 0.594              & 0.593                 & 0.612         \\ \hline
ProximalPhalanxOutlineAgeGroup & 0.833        & 0.835           & 0.853           & 0.844              & 0.845             & 0.837                & 0.845              & 0.835                 & 0.883         \\ \hline
ProximalPhalanxOutlineCorrect  & 0.902        & 0.910           & 0.914           & 0.908              & 0.906             & 0.910                & 0.906              & 0.910                 & 0.918         \\ \hline
ProximalPhalanxTW              & 0.811        & 0.802           & 0.816           & 0.791              & 0.814             & 0.799                & 0.810              & 0.805                 & 0.815         \\ \hline
MoteStrain                     & 0.918        & 0.906           & 0.909           & 0.901              & 0.927             & 0.908                & 0.920              & 0.903                 & 0.950         \\ \hline
MedicalImages                  & 0.768        & 0.753           & 0.756           & 0.755              & 0.768             & 0.751                & 0.771              & 0.760                 & 0.792         \\ \hline
Strawberry                     & 0.964        & 0.965           & 0.964           & 0.962              & 0.963             & 0.965                & 0.966              & 0.966                 & 0.980         \\ \hline
ToeSegmentation1               & 0.975        & 0.967           & 0.965           & 0.964              & 0.971             & 0.965                & 0.970              & 0.964                 & 0.974         \\ \hline
Coffee                         & 1.000        & 1.000           & 1.000           & 1.000              & 1.000             & 1.000                & 1.000              & 1.000                 & 1.000         \\ \hline
Cricket\_X                     & 0.773        & 0.791           & 0.788           & 0.814              & 0.746             & 0.762                & 0.782              & 0.791                 & 0.821         \\ \hline
Cricket\_Y                     & 0.764        & 0.798           & 0.798           & 0.819              & 0.759             & 0.798                & 0.770              & 0.795                 & 0.826         \\ \hline
Cricket\_Z                     & 0.774        & 0.812           & 0.804           & 0.823              & 0.786             & 0.809                & 0.783              & 0.812                 & 0.836         \\ \hline
uWaveGestureLibrary\_X         & 0.757        & 0.773           & 0.763           & 0.782              & 0.832             & 0.834                & 0.766              & 0.774                 & 0.855         \\ \hline
uWaveGestureLibrary\_Y         & 0.649        & 0.674           & 0.652           & 0.682              & 0.727             & 0.745                & 0.668              & 0.676                 & 0.759         \\ \hline
uWaveGestureLibrary\_Z         & 0.737        & 0.745           & 0.736           & 0.747              & 0.777             & 0.773                & 0.740              & 0.745                 & 0.792         \\ \hline
ToeSegmentation2               & 0.903        & 0.929           & 0.899           & 0.928              & 0.905             & 0.933                & 0.905              & 0.927                 & 0.962         \\ \hline
DiatomSizeReduction            & 0.940        & 0.930           & 0.952           & 0.933              & 0.937             & 0.937                & 0.937              & 0.936                 & 0.977         \\ \hline
car                            & 0.913        & 0.932           & 0.888           & 0.907              & 0.917             & 0.902                & 0.915              & 0.927                 & 0.933         \\ \hline
CBF                            & 0.994        & 0.996           & 0.995           & 0.998              & 0.994             & 0.996                & 0.993              & 0.996                 & 1.000         \\ \hline
CinC\_ECG\_torso               & 0.832        & 0.847           & 0.809           & 0.843              & 0.890             & 0.890                & 0.830              & 0.848                 & 0.996         \\ \hline
Computers                      & 0.844        & 0.832           & 0.814           & 0.814              & 0.775             & 0.734                & 0.836              & 0.828                 & 0.848         \\ \hline
Earthquakes                    & 0.763        & 0.793           & 0.760           & 0.794              & 0.794             & 0.801                & 0.783              & 0.797                 & 0.801         \\ \hline
ECG5000                        & 0.939        & 0.941           & 0.940           & 0.940              & 0.942             & 0.942                & 0.940              & 0.941                 & 0.948         \\ \hline
ElectricDevices                & 0.714        & 0.705           & 0.722           & 0.705              & 0.742             & 0.732                & 0.717              & 0.719                 & 0.799         \\ \hline
FaceAll                        & 0.922        & 0.864           & 0.848           & 0.813              & 0.910             & 0.875                & 0.914              & 0.868                 & 0.929         \\ \hline
FaceFour                       & 0.934        & 0.953           & 0.950           & 0.953              & 0.874             & 0.876                & 0.934              & 0.955                 & 1.000         \\ \hline
FacesUCR                       & 0.933        & 0.952           & 0.942           & 0.946              & 0.917             & 0.932                & 0.934              & 0.951                 & 0.965         \\ \hline
Fish                           & 0.937        & 0.969           & 0.971           & 0.983              & 0.958             & 0.967                & 0.953              & 0.972                 & 0.994         \\ \hline
FordA                          & 0.919        & 0.924           & 0.921           & 0.928              & 0.918             & 0.931                & 0.915              & 0.924                 & 0.973         \\ \hline
FordB                          & 0.880        & 0.902           & 0.916           & 0.918              & 0.883             & 0.904                & 0.881              & 0.902                 & 0.917         \\ \hline
Gun\_Point                     & 1.000        & 1.000           & 0.997           & 1.000              & 0.995             & 0.998                & 1.000              & 1.000                 & 1.000         \\ \hline
Ham                            & 0.715        & 0.750           & 0.712           & 0.730              & 0.717             & 0.727                & 0.720              & 0.750                 & 0.781         \\ \hline
HandOutlines                   & 0.521        & 0.755           & 0.880           & 0.871              & 0.842             & 0.875                & 0.623              & 0.806                 & 0.960         \\ \hline
Haptics                        & 0.426        & 0.494           & 0.517           & 0.553              & 0.489             & 0.514                & 0.465              & 0.510                 & 0.551         \\ \hline
Herring                        & 0.634        & 0.703           & 0.614           & 0.661              & 0.641             & 0.698                & 0.647              & 0.727                 & 0.703         \\ \hline
InlineSkate                    & 0.374        & 0.423           & 0.482           & 0.432              & 0.465             & 0.446                & 0.424              & 0.427                 & 0.613         \\ \hline
LargeKitchenAppliances         & 0.890        & 0.895           & 0.903           & 0.897              & 0.685             & 0.744                & 0.897              & 0.897                 & 0.896         \\ \hline
Lighting2                      & 0.708        & 0.711           & 0.730           & 0.726              & 0.752             & 0.769                & 0.718              & 0.728                 & 0.885         \\ \hline
MALLAT                         & 0.963        & 0.966           & 0.938           & 0.961              & 0.963             & 0.961                & 0.966              & 0.966                 & 0.980         \\ \hline
Meat                           & 0.863        & 0.875           & 0.938           & 0.942              & 0.895             & 0.922                & 0.885              & 0.910                 & 1.000         \\ \hline
NonInvasiveFatalECG\_Thorax1   & 0.949        & 0.958           & 0.954           & 0.955              & 0.962             & 0.962                & 0.955              & 0.956                 & 0.962         \\ \hline
NonInvasiveFatalECG\_Thorax2   & 0.929        & 0.947           & 0.949           & 0.956              & 0.954             & 0.957                & 0.948              & 0.951                 & 0.969         \\ \hline
OliveOil                       & 0.533        & 0.720           & 0.827           & 0.847              & 0.593             & 0.770                & 0.587              & 0.767                 & 0.933         \\ \hline
OSULeaf                        & 0.979        & 0.970           & 0.974           & 0.965              & 0.895             & 0.907                & 0.979              & 0.971                 & 0.988         \\ \hline
PhalangesOutlinesCorrect       & 0.813        & 0.821           & 0.825           & 0.821              & 0.816             & 0.817                & 0.812              & 0.817                 & 0.854         \\ \hline
Phoneme                        & 0.336        & 0.345           & 0.354           & 0.345              & 0.252             & 0.265                & 0.340              & 0.343                 & 0.349         \\ \hline
plane                          & 1.000        & 1.000           & 1.000           & 1.000              & 1.000             & 1.000                & 1.000              & 1.000                 & 1.000         \\ \hline
RefrigerationDevices           & 0.510        & 0.528           & 0.555           & 0.534              & 0.466             & 0.480                & 0.507              & 0.525                 & 0.581         \\ \hline
ScreenType                     & 0.637        & 0.637           & 0.648           & 0.627              & 0.545             & 0.510                & 0.639              & 0.634                 & 0.707         \\ \hline
ShapeletSim                    & 0.956        & 0.926           & 0.948           & 0.874              & 0.966             & 0.953                & 0.927              & 0.921                 & 1.000         \\ \hline
ShapesAll                      & 0.885        & 0.903           & 0.912           & 0.917              & 0.890             & 0.904                & 0.884              & 0.902                 & 0.930         \\ \hline
SmallKitchenAppliances         & 0.734        & 0.759           & 0.769           & 0.735              & 0.610             & 0.599                & 0.766              & 0.757                 & 0.853         \\ \hline
StarlightCurves                & 0.964        & 0.975           & 0.976           & 0.977              & 0.965             & 0.974                & 0.964              & 0.975                 & 0.982         \\ \hline
SwedishLeaf                    & 0.969        & 0.966           & 0.960           & 0.960              & 0.971             & 0.968                & 0.968              & 0.968                 & 0.966         \\ \hline
Symbols                        & 0.973        & 0.983           & 0.972           & 0.980              & 0.963             & 0.963                & 0.976              & 0.984                 & 0.982         \\ \hline
synthetic\_control             & 0.985        & 0.999           & 0.994           & 0.998              & 0.978             & 0.999                & 0.980              & 0.999                 & 1.000         \\ \hline
Trace                          & 0.250        & 0.250           & 0.250           & 0.250              & 0.250             & 0.250                & 0.250              & 0.250                 & 1.000         \\ \hline
Two\_Patterns                  & 0.863        & 0.942           & 0.963           & 0.991              & 0.994             & 0.984                & 0.873              & 0.943                 & 1.000         \\ \hline
TwoLeadECG                     & 0.999        & 0.998           & 0.999           & 0.996              & 0.999             & 0.998                & 0.999              & 0.998                 & 1.000         \\ \hline
UWaveGestureLibraryAll         & 0.822        & 0.864           & 0.833           & 0.874              & 0.955             & 0.959                & 0.824              & 0.861                 & 0.976         \\ \hline
wafer                          & 0.997        & 0.999           & 0.995           & 0.997              & 0.998             & 0.999                & 0.997              & 0.998                 & 1.000         \\ \hline
Worms                          & 0.612        & 0.650           & 0.598           & 0.626              & 0.494             & 0.534                & 0.606              & 0.651                 & 0.805         \\ \hline
WormsTwoClass                  & 0.773        & 0.774           & 0.771           & 0.762              & 0.683             & 0.699                & 0.781              & 0.773                 & 0.831         \\ \hline
yoga                           & 0.860        & 0.879           & 0.878           & 0.888              & 0.903             & 0.904                & 0.879              & 0.883                 & 0.918         \\ \hline
\end{tabular}
\end{table*}
